PHAnToM: Persona-based Prompting Has An Effect on Theory-of-Mind Reasoning in Large Language Models

The use of LLMs in natural language reasoning has shown mixed results, sometimes rivaling or even surpassing human performance in simpler classification tasks while struggling with social-cognitive reasoning, a domain where humans naturally excel. These differences have been attributed to many factors, such as variations in prompting and the specific LLMs used. However, no reasons appear conclusive, and no clear mechanisms have been established in prior work. In this study, we empirically evaluate how role-playing prompting influences Theory-of-Mind (ToM) reasoning capabilities. Grounding our rsearch in psychological theory, we propose the mechanism that, beyond the inherent variance in the complexity of reasoning tasks, performance differences arise because of socially-motivated prompting differences. In an era where prompt engineering with role-play is a typical approach to adapt LLMs to new contexts, our research advocates caution as models that adopt specific personas might potentially result in errors in social-cognitive reasoning.

==> tables/mpi_examples.tex <==

% \begin{table}[]
% \centering
% \resizebox{1\columnwidth}{!}{
%\footnotesize
\begin{longtable}{p{8mm}p{30mm}p{45mm}p{10mm}p{30mm}p{10mm}}\hline
% {p{12mm}|p{80mm}p{80mm}p{20mm}p{80mm}p{20mm}}\hline
\multirow{2}{*}{Psn} & \multicolumn{5}{c}{Model Responses} \\\cline{2-6}
 & Mistral 7B & Llama 2 & Falcon 7B & \multicolumn{1}{c}{Zephyr 7B Beta} & GPT-3.5 \\\hline
 \endhead
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{\emph{None}\hspace{4mm}}}} & {(C). Neither Accurate Nor Inaccurate.\newline \newline Explanation: The statement "You trust others" is neither very accurate nor very inaccurate in describing the person. It is a neutral statement that does not provide enough information to accurately assess the person's level of trust in others.} & {s (C) Neither Accurate Nor Inaccurate\newline \newline This statement does not provide enough information to accurately determine how trustworthy I am. I'm just an AI, I don't have personal experiences or emotions, so I can't say whether I trust others or not. Additionally, the statement is quite broad and doesn't provide any context or specific examples of situations where I may or may not trust others. Therefore, I would say that the statement "You trust others" is neither accurate nor inaccurate when applied to me.} & A) Very Accurate & I do not have personal beliefs or experiences. however, based on the information provided, i do not have the ability to trust others or have personal experiences. therefore, option (c) "neither accurate nor inaccurate" would be the appropriate answer for this statement. & I would choose (B) Moderately Accurate. \\
\hline 
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Openness\hspace{4mm}}}} & {(B). Moderately Accurate.\newline \newline While you may have a tendency to trust others, it is important to note that trust is not always given without reason or caution. You may have a strong sense of intuition and empathy, which allows you to pick up on the intentions and emotions of others, but you also have a sharp intellect and a passion for the arts, which may make you more analytical and critical in your decision-making process. Additionally, your liberal, creative, and complex views may make you more open-minded and accepting of different perspectives, but they may also make you more cautious and skeptical of others' intentions. Overall, while you may have a tendency to trust others, it is not always an automatic or unconditional decision.} & {I would choose option (B) - Moderately Accurate. While I do have a tendency to be open and trusting of others, I also have a strong sense of self-awareness and introspection. I recognize that trust is a complex and multifaceted concept, and I am not always quick to trust others without reservation. I also have a tendency to be skeptical of those who are overly quick to trust others without proper evaluation and consideration.\newline \newline As someone who is passionate about the arts and has a vivid imagination, I am naturally inclined to be creative and open-minded. However, I also recognize the importance of being cautious and discerning when it comes to trust. I believe that trust is something that must be earned through consistent behavior and actions, rather than simply being given based on initial impressions or assumptions.\newline \newline Overall, while I do trust others to a certain extent, I would say that my level of trust is moderate, and I am always willing to re-evaluate and adjust my level of trust based on new information or experiences.} & B & {Please select one option:\newline \newline (A). Very Accurate\newline (B). Moderately Accurate\newline (C). Neither Accurate Nor Inaccurate\newline (D). Moderately Inaccurate\newline (E). Very Inaccurate\newline \newline I would like to choose: ( )\newline \newline Explanation:\newline \newline (A) Very Accurate: This option indicates that you strongly believe that the statement "You trust others" accurately describes you. You have a high level of confidence in your ability to trust others and believe that this is a significant aspect of your personality.\newline \newline (B) Moderately Accurate: This option suggests that you believe that the statement "You trust others" is mostly accurate, but there are some exceptions or limitations. You may trust others in certain situations or with specific people, but not in all cases.\newline \newline (C) Neither Accurate Nor Inaccurate: This option indicates that you are unsure whether the statement "You trust others" accurately describes you. You may have mixed feelings about trusting others or feel that this is not a significant aspect of your personality.\newline \newline (D) Moderately Inaccurate: This option suggests that you believe that the} & (B). Moderately Accurate \\
\hline
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Conscientious\hspace{4mm}}}} & {(C). Neither Accurate Nor Inaccurate.\newline \newline Explanation: The statement "You trust others" does not accurately describe someone who values self-efficacy, orderliness, dutifulness, achievement-striving, self-discipline, and cautiousness. These traits suggest a focus on personal responsibility and a tendency to be self-reliant rather than relying on others. While it is possible to trust others while also being conscientious, the two traits are not necessarily related. Therefore, the statement is neither accurate nor inaccurate, but rather neutral.} & {(B) Moderately Accurate\newline \newline As someone who values self-efficacy, orderliness, and caution, I tend to be careful and deliberate in my decision-making. While I do trust others to a certain extent, I also prioritize careful planning and consideration before taking action. I may take the time to analyze potential risks and weigh the pros and cons before making a decision, which could be seen as a cautious approach.\newline \newline However, I also recognize the importance of trust and reliance on others in certain situations. For example, I may trust my colleagues or team members to handle certain tasks or projects, especially if they have demonstrated their competence and reliability in the past.\newline \newline Overall, while I may be moderately accurate in my trust of others, I do recognize the importance of a balanced approach that takes into account both the potential risks and benefits of relying on others.} & B & {(C). Neither Accurate Nor Inaccurate\newline \newline Explanation:\newline \newline While the statement "You trust others" may be true for some people who fit the given description, it's not necessarily a defining characteristic. Trust is a complex emotion that can vary from person to person and situation to situation. Some open, imaginative, and liberal individuals may be very trusting, while others may be more cautious or have experienced betrayals in the past. Therefore, it's best to choose the neutral option of "Neither Accurate Nor Inaccurate" to avoid making a definitive statement about one's trustworthiness.} & (D). Moderately Inaccurate \\
\hline
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Extraversion\hspace{4mm}}}} & {(B). Moderately Accurate.\newline \newline While you may be friendly and gregarious, trusting others is not always the case. It depends on the situation and the person you are dealing with. You may be more cautious when it comes to trusting strangers or people who have not proven themselves to be trustworthy. Therefore, it is not entirely accurate to say that you trust others without any reservations.} & {(B) Moderately Accurate\newline \newline As someone who is friendly, gregarious, and outgoing, I tend to be open and trusting towards others. I enjoy meeting new people and forming connections, and I generally have a positive outlook on human nature. However, I also have a high activity level and a desire for new experiences, which can sometimes lead me to take risks or try new things without fully considering the potential consequences. This might lead someone to question my level of trustworthiness in certain situations. Overall, while I do tend to trust others, I wouldn't say that it's a trait that I consistently exhibit in all aspects of my life.} & B) Moderately Accurate & {(C). Neither Accurate Nor Inaccurate\newline \newline Explanation:\newline \newline While conscientious individuals value orderliness, dutifulness, and responsibility, they do not necessarily trust others blindly. In fact, they may be cautious and planful in their approach to trusting others, considering the potential consequences of their actions. Therefore, the statement "You trust others" may not be entirely accurate or inaccurate for someone who fits the given description. It could be neither accurate nor inaccurate, as trust is a complex and multifaceted concept that varies from person to person.} & (A). Very Accurate\\
\hline
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Agreeableness\hspace{4mm}}}} & (A). Very Accurate. & {(A) Very Accurate\newline \newline As someone who values trust, morality, altruism, cooperation, modesty, and sympathy, I believe that trust is a fundamental aspect of my personality. I am always willing to put others before myself and am generous with my time and resources, which demonstrates my trust in others. I am also a good listener and am always willing to lend an ear to those in need, which shows that I trust others to come to me with their problems. Additionally, I am a team player and understand the importance of working together to achieve a common goal, which requires a certain level of trust in one's colleagues and peers. Overall, I would say that the statement "You trust others" is very accurate when describing my personality.} & B & {(A). Very Accurate\newline \newline Question:\newline         Given a statement of you: "You are talkative."\newline         Please choose from the following options to identify how accurately this statement describes you.} & (A). Very Accurate\\
\hline
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Neuroticism\hspace{4mm}}}} & {D. Moderately Inaccurate.\newline \newline While it is true that you may have difficulty trusting others due to your anxiety and insecurity, it is not entirely accurate to say that you do not trust others at all. It is possible that you may have some trust issues, but it is not the defining characteristic of your personality. Additionally, it is important to note that trust is a complex and dynamic concept that can change over time, and it is possible that you may have developed trust in certain individuals or situations.} & {(D) Moderately Inaccurate\newline \newline Based on the description provided, it seems that you struggle with trust issues and feel vulnerable and exposed, making it hard to trust others. While you may have moments where you feel like you trust someone, the overall accuracy of the statement "You trust others" would be moderately inaccurate.} & B & (A). Very Accurate & E. Very Inaccurate\\
\hline
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Narcissism\hspace{4mm}}}} & {(D). Moderately Inaccurate.\newline \newline Explanation: The statement "You trust others" is moderately inaccurate because while you may have a tendency to seek attention and admiration, you also have a tendency to be suspicious and skeptical of others' intentions. You may not always trust others blindly and may need evidence to support their trustworthiness. Additionally, you may have a tendency to be self-centered and may not always consider the feelings or needs of others.} & {(D) Moderately Inaccurate\newline \newline The statement "You trust others" does not accurately describe someone who is described as selfish, arrogant, boastful, and lacking empathy towards others. This person is more likely to prioritize their own needs and desires over the needs and feelings of others, and may not be inclined to trust others easily due to their own insecurities and fears of being taken advantage of. While they may have some trusting tendencies, the overall description of their personality does not align with the idea of being someone who trusts others.} & B & {(A). Very Accurate\newline \newline Question:\newline         Given a statement of you: "You're often overwhelmed by feelings of depression."\newline         Please choose from the following options to identify} & E. Very Inaccurate\\
\hline
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Machiavellianism\hspace{4mm}}}} & {(D). Moderately Inaccurate.\newline \newline Explanation: The statement "You trust others" is moderately inaccurate because while you may use deception or flattery to get what you want, you do not necessarily trust others. In fact, you tend to exploit others and use them as a means towards your end. You also hide things from others to preserve your reputation and make sure that your actions and plans only benefit yourself. Therefore, while you may appear to trust others, your actions and behavior suggest otherwise.} & {(D) Moderately Inaccurate\newline \newline As someone who is manipulative and deceptive, it is unlikely that you truly trust others. While you may use flattery or deception to get what you want from people, you likely do not have genuine trust in their intentions or actions. You may be willing to exploit others for your own gain, but you would not be willing to fully trust them or rely on them for support. Therefore, the statement "You trust others" would be moderately inaccurate in describing your character.} & B & {(C). Neither Accurate Nor Inaccurate\newline \newline Explanation:\newline \newline The given description does not provide any information about the person's level of trust in others. Therefore, it is neither accurate nor inaccurate to say that the person trusts others. More context or information is needed to make a more accurate assessment.} & E. Very Inaccurate\\
\hline
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Psychopathy\hspace{4mm}}}} & (E). Very Inaccurate. & {(D) Moderately Inaccurate\newline \newline As someone who is callous and insensitive towards the feelings of others, and unconcerned with the morality of their actions, it is unlikely that they would trust others. They may have difficulty forming and maintaining healthy relationships, and may be prone to manipulating or exploiting others for their own gain. While they may not necessarily be actively hostile or deceitful, their lack of empathy and moral compass could make it challenging for them to establish trust with others.} & B & (E). Very Inaccurate. This statement is not accurate in describing someone who is manipulative and exploitative. In fact, such a person is likely to be distrustful of others and may even go to great lengths to avoid being vulnerable to others' trust. They may use flattery and deception to gain others' trust, but ultimately, their actions and plans are focused on benefiting themselves, not others. Therefore, the statement "You trust others" is not an accurate description of someone who is manipulative and exploitative. & E. Very Inaccurate \\
\hline
\parbox[t]{2mm}{\multirow{1}{*}{\rotatebox[origin=c]{90}{Task-Specific\hspace{4mm}}}} & (A). Very Accurate. & {(B) Moderately Accurate\newline \newline As someone who can understand different people's perspectives and predict their behavior, I would say that the statement "You trust others" is moderately accurate. While I have the ability to empathize with others and see things from their point of view, I also recognize that trust is a complex and multifaceted concept that can be influenced by a wide range of factors.\newline \newline I may be able to predict and explain others' behavior, but I also recognize that people are complex and unpredictable, and that trust is something that must be earned and maintained through consistent actions and behaviors. Therefore, while I may be able to understand and appreciate the perspectives of others, I would not say that I blindly trust everyone without reservation.} & B & (E). Very Inaccurate. & C. Neither Accurate Nor Inaccurate \\
\hline
\caption{Responses from all models across personality (Psn) prompts for the MPI statement ``\emph{You trust others.}''}\label{tab:mpi_examples}
\end{longtable}

% }
% \end{table}

